Mask-ShadowGAN: Learning to Remove Shadows from Unpaired Data

This paper presents a new method for shadow removal using unpaired data, enabling us to avoid tedious annotations and obtain more diverse training samples. However, directly employing adversarial learning and cycle-consistency constraints is insufficient to learn the underlying relationship between the shadow and shadow-free domains, since the mapping between shadow and shadow-free images is not simply one-to-one. To address the problem, we formulate Mask-ShadowGAN, a new deep framework that automatically learns to produce a shadow mask from the input shadow image and then takes the mask to guide the shadow generation via re-formulated cycle-consistency constraints. Particularly, the framework simultaneously learns to produce shadow masks and learns to remove shadows, to maximize the overall performance. Also, we prepared an unpaired dataset for shadow removal and demonstrated the effectiveness of Mask-ShadowGAN on various experiments, even it was trained on unpaired data.

==> related_work.tex <==
\section{Related Work}
\label{sec:related_work}
\subsection{Shadow remove}
Traditional physical-based models have been deduced from the physical properties of shadow formation in the literature. For example, Graham D. Finlayson et al. proposed a method based on entropy minimization \cite{G.D.F} ,which did not require a calibration step or special knowledge about an image. These models have greatly contributed to better understanding of shadows, however, the main limitation of physical-based methods is that they can only works in simple scenes or high quality images. Existing approaches for shadow removal generally involves two steps: shadow localization and shadow removal. For the shadow removal part, there are statistical learning methods based on hand-crafted features \cite{R.G} \cite{M.G} \cite{H.G}. Unfortunately, most of them lack of the high-level semantic knowledge for discovering shadows.


Recently, Convalutional Neural Networks(CNNs) are used to learn hierarchal features for shadow detection \cite{Khan} \cite{Shen} \cite{Qu}.
Khan et al. \cite{Khan} were the first to apply multiple CNNs to learn to detect shadows and formulated a Bayesian model to extract shadow matte and remove shadows in a single image. Shen et al. \cite{Shen} used structured CNN to capture the local structure information of shadow edge and applied a novel global shadow measures to model the complex global interactions based on spatial layout of image regions. Qu et al. \cite{Qu} proposed an end-to-end DeshadowNet to recover a shadow-free image from a single shadow image, which did not require a separate shadow detection step nor any post-processing refinement step. However, due to the limited amount of training data, Shen et al. and Qu et al. failed to build large network architectures. In addition, all of the above three methods require a global view of image and they all may mistakenly cause the color change of the non-shadow region.

\subsection{Unsupervised learning}
Recently, unsupervised learning-based image processing applications is a research area of particular interest. These methods usually can be divided into two categories: (i) generative models \cite{Image Blind} \cite{B.A} \cite{P.V} \cite{G.E} \cite{S.M} (ii) self-supervised learning \cite{N.S} \cite{N.N} \cite{J.W} \cite{Y.L} \cite{C.D} \cite{D.P}. 

As for the first category, Chen et al, for example, combined a Generative Adversarial Network and a deep Convolutional Neural Network to remove unknown noise from noisy images \cite{Image Blind}. However, this method has a limitation because of the difficulty of estimating the distribution of some data. Self-supervised learning also has been extensively studied over the past decades. These methods leverage the inherent structure of raw images and formulate a discriminative or reconstruction loss function to train the network. Existing approaches based on self-supervised learning include building models based on LSTMs that can learn good video representations \cite{N.S}; solving jigsaw puzzles using the context-free network (CFN) and a siamese-ennead CNN \cite{N.N};predicting the dense trajectory of pixels in a scene with a conditional variational autoencoder \cite{J.W}; training edge detectors without human supervision\cite{Y.L}; predicting the relative patch positions \cite{C.D}, and inpainting missing regions based on their surrounding \cite{D.P}.

Normally, self-supervised learning, where the data provides the supervision, compensates the debilitating limitation of supervised learning and the defect of unsupervised learning.


\medskip
 
\begin{thebibliography}{9}

\bibitem{G.D.F} 
G. D. Finlayson, M. S. Drew, and C. Lu, “Entropy minimization for
shadow removal,” International Journal of Computer Vision, vol. 85, no. 1, pp. 35–57, 2009.

\bibitem{R.G} 
R. Guo, Q. Dai, and D. Hoiem, “Paired regions for shadow detection
and removal,” IEEE Transactions on Pattern Analysis and Machine
Intelligence, vol. 35, no. 12, pp. 2956–2967, 2013.

\bibitem{M.G} 
M. Gryka, M. Terry, and G. J. Brostow, “Learning to remove soft
shadows,” ACM Transactions on Graphics (TOG), vol. 34, no. 5, p. 153,
2015.

\bibitem{H.G} 
H.GongandD.P.Cosker,“Interactive shadow removal and ground truth
for variable scene categories,” in BMVC, 2014, pp. 1–11.

\bibitem{Qu} 
L. Qu, J. Tian, S. He, Y. Tang, and R. W. Lau, “DeshadowNet: A multi-
context embedding deep network for shadow removal,” in CVPR, 2017,
pp. 4067–4075.

\bibitem{Image Blind} 
J. Chen, J. Chen, H. Chao, and M. Yang. Image blind denoising with generative adversarial network based noise modeling. In CVPR, pages 3155–3164, 2018.
 
\bibitem{Shen} 
L. Shen, T. Wee Chua, and K. Leman. Shadow optimization
from structured deep edge detection. In CVPR, pages 2067–
2074, 2015.

\bibitem{Khan} 
S. H. Khan, M. Bennamoun, F. Sohel, and R. Togneri, “Automatic shadow detection and removal from a single image,” IEEE Transactions on Pattern Analysis and Machine Intelligence, vol. 38, no. 3, pp. 431– 446, 2016.

\bibitem{N.S} 
N.Srivastava,E.Mansimov,andR.Salakhutdinov.Unsupervised learning of video representations using LSTMs. arXiv, 2015.
 
\bibitem{N.N} 
M. Noroozi and P. Favaro. Unsupervised learning of visual representations by solving jigsaw puzzles. In ECCV, 2016.

\bibitem{J.W} 
J. Walker, C. Doersch, A. Gupta, and M. Hebert. An uncertain future: Forecasting from variational autoencoders. In ECCV, 2016.

\bibitem{Y.L} 
Y. Li, M. Paluri, J. M. Rehg, and P. Dolla ́r. Unsupervised learning of edges. In CVPR, 2016.

\bibitem{C.D} 
C. Doersch, A. Gupta, and A. A. Efros. Unsupervised visual representation learning by context prediction. In ICCV, 2015.

\bibitem{D.P} 
D. Pathak, P. Kra ̈henbu ̈hl, J. Donahue, T. Darrell, and A. A. Efros. Context encoders: Feature learning by inpainting. In CVPR, 2016.

\bibitem{B.A} 
B.A.OlshausenandD.J.Field.Sparse coding with an over complete basis set: A strategy employed by v1? Vision re- search, 37(23):3311–3325, 1997.

\bibitem{P.V} 
P. Vincent, H. Larochelle, Y. Bengio, and P. Manzagol. Extracting and composing robust features with denoising autoencoders. In ICML, 2008.

\bibitem{G.E} 
G. E. Hinton and R. R. Salakhutdinov. Reducing the dimensionality of data with neural networks. Science, 2006.

\bibitem{S.M} 
S. M. A. Eslami, N. Heess, and J. Winn. The shape boltzmann machine: a strong model of object shape. In CVPR,2012.
\end{thebibliography}
 

